A Model Predictive Control Framework for Improving Risk-Tolerance of Manufacturing Systems

The need for control strategies that can address dynamic system uncertainty is becoming increasingly important. In this work, we propose a Model Predictive Control by quantifying the risk of failure in our system model. The proposed control scheme uses a Priced Timed Automata representation of the manufacturing system to promote the fail-safe operation of systems under uncertainties. The proposed method ensures that in case of unforeseen failure(s), the optimization-based control strategy can still achieve the manufacturing system objective. In addition, the proposed strategy establishes a trade-off between minimizing the cost and reducing failure risk to allow the manufacturing system to function effectively in the presence of uncertainties. An example from manufacturing systems is presented to show the application of the proposed control strategy.

==> figure-case-study-paths.tex <==
\begin{figure*}[bt]
    \begin{center}
    \begin{adjustbox}{scale=0.8}
    \begin{tikzpicture}[node distance = 2cm, on grid,>={Stealth[inset=0pt,length=6pt,angle'=28,round]},fill_fraction/.style n args={2}{path picture={
            \fill[#1] (path picture bounding box.center) -- (path picture bounding box.south)  arc [start angle=-90, delta angle=-100, radius=1] -- cycle;
            \fill[#2] (path picture bounding box.center) -- (path picture bounding box.south)  arc [start angle=-90, delta angle=100, radius=1] -- cycle;
            }}
    ,fill_fractiontwo/.style n args={1}{path picture={
            \fill[#1] (path picture bounding box.center) -- (path picture bounding box.south)  arc [start angle=-90, delta angle=-180, radius=1] -- cycle;
            }}
            ]

    \begin{customlegend}[legend style={at={(6,-4)},anchor=south},legend columns=-1,legend style={column sep=1ex},legend entries={PCM PTA-MPC,CB PTA-MPC,PTA-MPC,Failed State}]
    \addlegendimage{black,only marks, mark=*, fill=blue!40,style={scale=4}}
    \addlegendimage{black,only marks, mark=*, fill=green!30,style={scale=4}}
    \addlegendimage{black,only marks, mark=*, fill=magenta!50,style={scale=4}}
    \addlegendimage{black,only marks, mark=*, pattern=north west lines, pattern color=black,style={scale=4}}
   \end{customlegend};
   
    \node[state, initial, opacity=1, fill= green!30,fill_fraction={blue!40}{magenta!50}] (q1) {$q^{1}$};
    \node[state,fill=blue!40] at (1,-2.5) (q2) {$q^{2}$};
    \node[state, right of=q2,fill=blue!40] (q3) {$q^{3}$};
    \node[state, right of=q3,fill=blue!40] (q4) {$q^{4}$};
    \node[state, opacity=1, right of=q4,pattern=north west lines, pattern color=black] (q5) {$q^{5}$};
    \node[state, right of=q5] (q6) {$q^{6}$};
    \node[state, right of=q6] (q7) {$q^{7}$};
    
    
    
    \node[state, fill=magenta!50] at (2,0) (q9) {$q^9$};
    \node[state, right of=q9,pattern=north west lines, pattern color=black] (q10) {$q^{10}$};
    \node[state, right of=q10,fill=blue!40, fill_fractiontwo={green!30}] (q11) {$q^{11}$};
    \node[state, right of=q11,fill=blue!40, fill_fractiontwo={green!30}] (q12) {$q^{12}$};
    \node[state, right of=q12,fill=blue!40, fill_fractiontwo={green!30}] (q13) {$q^{13}$};
    \node[state,fill=blue!40, fill_fractiontwo={green!30}, right of=q13] (q8) {$q^{8}$};
    
    \node[state, fill= green!30] at (1,2.5) (q14) {$q^{14}$};
    \node[state, right of=q14, fill= green!30] (q15) {$q^{15}$};
    \node[state, right of=q15, fill= green!30] (q16) {$q^{16}$};
    \node[state, right of=q16,pattern=north west lines, pattern color=black] (q17) {$q^{17}$};
    \node[state, right of=q17] (q18) {$q^{18}$};
    \node[state, right of=q18] (q19) {$q^{19}$};
    
    \node[state,fill=red!20, densely dashed] at (3,-1.25) (q20) {$q^{20}$};
    \node[state,fill=blue!40, densely dashed] at (7,-1.25) (q21) {$q^{21}$};
    \node[state,fill=red!20, densely dashed] at (11,-1.25) (q22) {$q^{22}$};
    \node[state,fill=red!20, densely dashed] at (2,1.25) (q23) {$q^{23}$};
    \node[state,fill=green!30, densely dashed] at (5,1.25) (q24) {$q^{24}$};
    \node[state,fill=red!20, densely dashed] at (7,1.25) (q25) {$q^{25}$};
    \node[state,fill=red!20, densely dashed] at (11,1.25) (q26) {$q^{26}$};

 \draw 
    
   (q1) edge[bend right] node [below left]{} (q2)
   (q2) edge node [below] {} (q3)
   (q3) edge node [below]{} (q4)
%   (q4) edge node [below]{} (q5)
%   (q5) edge node [below]{} (q6)
   (q6) edge node [below]{} (q7)
   (q7) edge[bend right] node [below right] {} (q8)
   
   (q1) edge node [above]{} (q9)
%   (q9) edge node [above]{} (q10)
%   (q10) edge node [above]{} (q11)
   (q11) edge node [above]{} (q12)
   (q12) edge node [above]{} (q13)
   (q13) edge node [above]{} (q8)
   
   (q1) edge[bend left] node [below left]{} (q14)
   (q14) edge node [above]{} (q15)
   (q15) edge node [above]{} (q16)
%   (q16) edge node [above]{} (q17)
%   (q17) edge node [above]{} (q18)
   (q18) edge node [above]{} (q19)
   (q19) edge[bend left] node [above right]{} (q8)
   
   (q2) edge[bend right, densely dashed] node [above left]{} (q20)
   (q20) edge[bend right, densely dashed] node [above left]{} (q9)
   (q4) edge[bend right, densely dashed] node [right]{} (q21)
   (q21) edge[bend right, densely dashed] node [right]{} (q11)
   (q6) edge[bend right, densely dashed] node [right]{} (q22)
   (q22) edge[bend right, densely dashed] node [right]{} (q13)
   (q15) edge[bend right, densely dashed] node [right]{} (q23)
%   (q23) edge[bend right, densely dashed] node [right]{} (q10)
   (q15) edge[bend left, densely dashed] node [right]{} (q24)
   (q24) edge[bend right, densely dashed] node [right]{} (q11)
   (q18) edge[bend right=10, densely dashed] node [above right]{} (q25)
   (q25) edge[bend right, densely dashed] node [above right]{} (q12)
   (q18) edge[bend left, densely dashed] node [above right]{} (q26)
   (q26) edge[bend left, densely dashed] node [above right]{} (q13);
    \end{tikzpicture}
    \end{adjustbox}
    \end{center}
    \caption{The solution for PCM risk-averse PTA-MPC (purple), Centrality-based risk-averse PTA-MPC (green), and regular PTA-MPC (red) under unpredictable state failure (hashed black) for a sample production line.}
    \label{figure-samplePTAunderfailure}
\end{figure*}

